Estimating Geographic Spillover Effects of COVID-19 Policies From Large-Scale Mobility Networks

Many policies in the US are determined locally, e.g., at the county-level. Local policy regimes provide flexibility between regions, but may become less effective in the presence of geographic spillovers, where populations circumvent local restrictions by traveling to less restricted regions nearby. Due to the endogenous nature of policymaking, there have been few opportunities to reliably estimate causal spillover effects or evaluate their impact on local policies. In this work, we identify a novel setting and develop a suitable methodology that allow us to make unconfounded estimates of spillover effects of local policies. Focusing on California's Blueprint for a Safer Economy, we leverage how county-level mobility restrictions were deterministically set by public COVID-19 severity statistics, enabling a regression discontinuity design framework to estimate spillovers between counties. We estimate these effects using a mobility network with billions of timestamped edges and find significant spillover movement, with larger effects in retail, eating places, and gyms. Contrasting local and global policy regimes, our spillover estimates suggest that county-level restrictions are only 54% as effective as statewide restrictions at reducing mobility. However, an intermediate strategy of macro-county restrictions -- where we optimize county partitions by solving a minimum k-cut problem on a graph weighted by our spillover estimates -- can recover over 90% of statewide mobility reductions, while maintaining substantial flexibility between counties.

==> Spillovers paper - arxiv/acks.tex <==
\section*{Acknowledgements}
S. C. was supported in part by an NSF Graduate Research Fellowship and the Meta PhD Fellowship. The authors thank Emma Pierson, Martin Saveski, Hamed Nilforoshan, and anonymous reviewers for helpful comments and discussions.

==> Spillovers paper - arxiv/causal.tex <==
\section{Causal framework} \label{sec:causal}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/fig2.pdf}
    \caption{Visualizing our $Z$ variable. (a) $Z$ almost perfectly separates counties in the purple and red tiers. 
    (b) Triggering patterns for $Z$ (among large counties compliers).
    (c) Cross-county mobility vs $Z$. 
    All source counties are in purple ($0 \leq Z \leq 5$) and the x-axis represents the target county's $Z$. Black lines represent linear fits and dots are average outcomes per bin (size represents the number of data points in the bin). We observe a discontuinity at $Z=0$, when the target county changes from purple to red.}
    \label{fig:z_viz}
\end{figure*}

To capture spillovers, our objective is to estimate the effect of \textit{pairwise} tiers on cross-county mobility. 
% More specifically, given a unit $(i, j, w)$, indexing CBG $c_i$, POI $p_j$, and week $w$, we estimate the effect of the treatment $(T_{iw}, T_{jw})$, the CBG and POI's tiers, on the mobility outcome $Y_{ijw}$, the number of visits from $c_i$ to $p_j$ in week $w$. 
The key to our causal framework is that we can utilize RD design, which is widely recognized as ``one of the most credible non-experimental strategies for the analysis of causal effects'' \citep{cattaneo2020intro}. In a typical RD design, units are assigned to the treatment or control condition according to an exogenously determined threshold of a single continuous variable, known as the assignment variable (or running or forcing variable). 
Researchers can then compare the outcomes for units just below the threshold to units just above the threshold to estimate the \textit{local} causal effect of treatment.
A primary advantage of RD design is that it achieves unconfoundedness, without needing to control for all possible confounders. 
This is because the unconfoundedness assumption is met: treatment assignment is conditionally independent of potential outcomes, given covariates \citep{imbens2008rd}. 
This assumption is clearly met in RD design, since treatment assignment is determined by the assignment variable, and so, conditioned on covariates, there is no variation in treatment. 

Our problem generally fits RD design, since Blueprint tiers were assigned at the thresholds of continuous COVID-19 metrics. We focus on the threshold between the purple and red tiers, since they were the adjacent pair with the most support. 
However, we need to extend generic RD design in two ways: (1) to account for multiple assignment variables, since tiers were assigned based on numerous COVID-19 metrics, (2) to account for multiple treatment conditions, since we are considering pairwise tiers as our treatment. We describe our approach in the following sections.

\paragraph{Assigning Blueprint tiers.}
First, let us focus on the problem of determining a single county's tier, $T_{iw}$, from its COVID-19 metrics.
Tier assignments depended on three metrics: adjusted case rate, test positivity rate, and a health equity metric, which was the test positivity rate in the most disadvantaged quartile of neighborhoods \citep{cdph2021healtheq}.
To advance to a less restricted tier, counties needed to meet the criteria for movement for two consecutive weeks \citep{cdph2021blueprint}. For a large county (population over 106,000), the criteria to move from purple to red could be met in two ways: (1) by meeting the thresholds for the red tier for all three metrics, (2) by meeting the thresholds for test positivity and health equity for the \textit{orange} tier, thus exchanging adjusted case rate for more stringent thresholds on the other two.
\extended{Small counties (population under 106,000) only had one possible path, which was to meet the adjusted case rate and test positivity thresholds for the red tier.}
Small counties were not required to meet the health equity thresholds, but needed to demonstrate their commitment to equity through other plans \citep{cdph2021healtheq}.
For most of the duration of the Blueprint, the purple-red threshold for adjusted case rate was 7 per 100,000 and 8\% for test positivity and health equity (and 5\% for the red-orange threshold). The purple-red threshold for adjusted case rate was increased to 10 per 100,000 on March 12, 2021, after 2 million vaccines had been administered statewide \citep{calmatters2021vaccinegoal}.

\paragraph{Constructing a single assignment variable $Z$.}
We take a \textit{centering} approach to RD design with multiple assignment variables \citep{wong2013centering}. 
That is, we first center each of the assignment variables by subtracting their respective thresholds, then apply min/max aggregations to the centered variables in order to construct a new assignment variable $Z$ that can singly determine a unit's treatment.
More formally, we design a function $f: \mathbb{R}^m \rightarrow \mathbb{R}$ that maps a county’s $m$ COVID-19 metrics to a single continuous variable, $Z_{iw}$. For a large county, the $m$ metrics include the county's adjusted case rate ($CR$), test positivity ($TP$), and health equity metric ($HE$) from the preceding two weeks; for a small county, only adjusted case rate and test positivity. Our mapping $f$ satisfies the key property that $Z_{iw} < 0$ if and only if the county was assigned to the red tier.

Let $CR_{iw}^{\textrm{red}}$ represent the adjusted case rate for the county in week $w$ with the purple-red threshold subtracted, and let us define other terms similarly. We construct $Z_{iw}$ for large counties as follows:
\begin{align}
    Z_{1iw} &= \max(CR_{iw}^{\textrm{red}}, TP_{iw}^{\textrm{red}}, HE_{iw}^{\textrm{red}}, CR_{iw-1}^{\textrm{red}}, TP_{iw-1}^{\textrm{red}}, HE_{iw-1}^{\textrm{red}})\\
    Z_{2iw} &= \max(TP_{iw}^{\textrm{orange}}, HE_{iw}^{\textrm{orange}}, TP_{iw-1}^{\textrm{orange}}, HE_{iw-1}^{\textrm{orange}})\\
    Z_{iw} &= \min(Z_{1iw}, Z_{2iw}).
\end{align}
For small counties, we only have
\begin{align}
    Z_{iw} &= \max(CR_{iw}^{\textrm{red}}, TP_{iw}^{\textrm{red}}, CR_{iw-1}^{\textrm{red}}, TP_{iw-1}^{\textrm{red}}).
\end{align}
In Figure \ref{fig:z_viz}a, we show that our new $Z$ variable almost perfectly separates the counties in the purple and red tiers. 
Over the 9-week period from February 1 to March 29, 2021, there were 480 counties/weeks in the purple or red tier, and 471 of them follow that $Z_{iw} < 0$ if and only if the county is in the red tier. 
We manually check the non-compliers and find that they were cases of counties, mostly small, that were allowed to remain in the red tier upon special request, as noted in the CDPH documentation.

To interpret our new $Z$ variable, we also analyze its ``triggering'' patterns; that is, for each min/max aggregation, which input is the minimum or maximum (Figure \ref{fig:z_viz}b). 
\extended{Since $Z < 0$ moves the county into the red (less restricted) tier, a maximum can be interpreted as holding the county back and a minimum as improving the county's prospects.}
For large counties, we find that the most frequent maximum for the first criteria $Z_1$ is the adjusted case rate from week $w-1$. For the second criteria $Z_2$, the most frequent maximum is the health equity metric from week $w-1$. This reflects trends from this time period: COVID-19 severity was improving over time, so week $w-1$ tended to have higher rates than week $w$, and health equity (i.e., test positivity in the most disadvantaged quartile) tended to be worse than the overall test positivity. 
Interestingly, we also find that $Z_2$ triggers more often than $Z_1$, when taking the minimum between them. This indicates that this alternative path---meeting more stringent test positivity and health equity thresholds and dropping adjusted case rate---substantially helped counties move toward less restricted tiers.

\paragraph{RD design with pairwise treatments.}
We can now formulate an RD design problem where treatment (purple/red tier) is assigned at the threshold of a single continuous variable ($Z$). Since we are interested in spillover effects in this work, we use \textit{cross-county} mobility as our outcome. However, our RD framework is general and could be applied to study the effects of Blueprint tiers on a variety of outcomes, such as mask-wearing rates, vaccination rates, and COVID-19 cases and deaths.

With cross-county mobility as our outcome, our treatment becomes pairwise to capture the tier of each county, and we have four treatment conditions: $PP, PR, RP$ and $RR$, where $P$ and $R$ represent the purple and red tiers, respectively.
We are particularly interested in the difference between $PP$ and $PR$, since this difference indicates whether individuals from a restricted county will increase their visits to another county when that other county becomes less restricted.
In Figure \ref{fig:z_viz}c, we illustrate this comparison. We consider all source counties that were in the purple tier and plot their mobility to target counties that were either in the purple or red tier. The x-axis represents $Z$ for the target county, so that the region to the left of $Z=0$ represents the $PR$ condition and the region to the right represents $PP$. We see a discontinuity in visits at $Z=0$, indicating that there is indeed a local effect on cross-county visits when a neighboring county changes from more to less restricted.
% These plots suggest that populations were reacting to changes in tier, both within a county and in adjacent counties. 
In the following section, we estimate this effect more precisely by defining a zero-inflated Poisson regression model that we fit to the rich CBG-POI mobility network with covariates.

\paragraph{Poisson regression model.}
We define a Poisson regression model to describe visits from CBGs to POIs. 
For a given CBG $c_i$, POI $p_j$, and week $w$, the Poisson rate $\lambda_{ijw}$ is
\begin{align}
    \lambda_{ijw} &= \exp(\beta_0 + \beta_1 Z_{iw} + \beta_2 Z_{jw} +  \mathbf{\beta_3}^T\mathbf{X}_{ijw} + \beta_{T_{iw}, T_{jw}}),
\end{align}
where the $\beta$ terms are model parameters, $Z_{iw}$ and $Z_{jw}$ represent the $Z$ variables for $c_i$'s and $p_j$'s counties in this week, $T_{iw}$ and $T_{jw}$ describe their respective tiers, and $\mathbf{X}_{ij}$ contains other covariates. Those covariates include the distance between the POI and CBG, SafeGraph's CBG device count in that week, CBG demographics from US Census, and POI attributes (area in square feet, NAICS code).
Spillover effects are captured in the difference between the $\beta_{T_{iw}, T_{jw}}$ terms: for example, $\exp(\beta_{PR} - \beta_{PP})$ represents the multiplicative increase in visits when a POI changes from the purple to red tier, while the CBG remains in purple.
\extended{To capture heterogeneous treatment effects, we learn separate $\beta_{T_{iw}, T_{jw}}$'s for different POI groups (Table \ref{tab:poi-groups}). We also learn separate $\beta_1$'s and $\beta_2$'s for our four different constructions of $Z$ that reflect two binary dimensions: 1) large vs. small county, 2) before vs. after March 12, 2021, when the statewide vaccine goal was met and the adjusted case rate threshold was increased.}

The CBG-POI network is very large, with billions of edges, but over 99\% of the edges represent zero visits. Thus, we zero-inflate our Poisson model, based on the notion that observed zeros in zero-heavy data may represent actual preferences, but could also reflect lack of exposure \citep{liu2017zeroinf}, i.e., the CBG had never heard of the POI. We represent each number of visits $Y_{ijw}$ as drawn from a mixture of a Poisson($\lambda_{ijw}$) and $\delta_0$ (a point mass on 0), with mixing parameter $\pi_{ij}$. We assume the likelihood of exposure is inversely proportional to the distance $d_{ij}$ between the CBG and POI and define $\pi_{ij} = \frac{1}{1 + \alpha_1 d_{ij}^{\alpha_2}}$, where the $\alpha$ terms are learned.
Then, our generative model for $Y_{ijw}$ is
\begin{align}
    b_{ijw} &\sim \textrm{Bern}(\pi_{ij}) \\
    Y_{ijw} &\sim \begin{cases}
            \delta_0\textrm{ if $b_{ijw} = 0$,}\\
            \textrm{Poisson}(\lambda_{ijq}),\textrm{ otherwise.}
        \end{cases} 
\end{align}
In this mixture, the likelihood of a single data point given model parameters $\theta$ is
\begin{align}
    \Pr(Y_{ijw} = y | \theta) = \begin{cases}
        (1 - \pi_{ij}) + \pi_{ij} e^{-\lambda_{ijw}},\textrm{ if $y = 0$}\\
        \pi_{ij} \frac{\lambda_{ijw}^y e^{-\lambda_{ijw}}}{y!},\textrm{ otherwise.}\\
    \end{cases}
\end{align}
We fit our model using gradient descent, with negative log likelihood as our model loss.
% $\mathcal{L}$:
% \begin{align}
%     \mathcal{L}(\theta) &= -\sum_{i, j, w } \ln(\Pr(Y_{ijw} = y_{ijw} | \theta)).
% \end{align}

\paragraph{Data filtering and bandwidth selection.}
We focus our experiments on the 9-week period following the Regional Stay-At-Home Order, during which we could almost perfectly separate the purple and red tiers with our $Z$ variable (Figure \ref{fig:z_viz}a). 
\extended{We keep all CBGs with at least 50 non-zero visits (to any POIs) during this period and POIs with at least 30 non-zero visits (from any CBGs), so that we focus on CBGs and POIs for which SafeGraph has more reliable coverage; this filtering leaves 22,972 CBGs and 128,655 POIs.}
Due to the specifics of our RD-based analysis, we cannot keep every CBG-POI pair from every week. 
First, we do not fit the model on data from the week of March 8, 2021, since the purple-red threshold for adjusted case rate was changed in the middle of the week (due to the statewide vaccine goal being met). 
In the remaining 8 weeks, we keep all data points that meet the following criteria:
\begin{itemize}
    \item CBG $c_i$ and POI $p_j$ lie in adjacent counties,
    \item $T_{iw}$ and $T_{jw}$ are both in the purple or red tier,
    \item Both are compliers, i.e., $T_{iw}$ is red if and only if $Z_{iw} < 0$, and likewise for $T_{jw}$,
    \item $Z_{iw}$ and $Z_{jw}$ both lie within a bandwidth $h$ of 0.
\end{itemize}
\extended{In total over the 8 weeks, we keep 1.4 billion data points after filtering (Table \ref{tab:data_size}).} 

We only keep data points that fall within the bandwidth since our goal is to estimate the \textit{local} effect of changing tier pairs at the purple-red threshold ($Z=0$). 
By requiring both $Z_{iw}$ and $Z_{jw}$ to fall within the bandwidth, we interpret our resulting parameters as estimated effects at the \textit{joint} cutoff, when both the CBG and the POI are at the threshold.\footnote{Alternatively, RD design with multiple assignment variables can estimate effects along the threshold frontiers, i.e., varying one assignment variable while fixing the other one at its threshold \citep{papay2011multiple}. For simplicity, we focus on effects at the joint threshold.}
Bandwidth selection introduces a bias-variance trade-off, with larger bandwidths corresponding to greater bias but reduced variance. We err on the side of larger bandwidths in this work, out of concern for variance. Even though we have over a billion data points, our assignment variable $Z$ only varies at the level of counties and, thus, bandwidths that are too small could lead to very few counties represented, particularly for the $PR$ or $RP$ treatment conditions, which appear less often. We choose $h=5$, which keeps most of the counties in the red tier, but drops many of the counties in purple (Figure \ref{fig:z_viz}a). 
We show in the Appendix that each treatment condition is well-represented at this bandwidth, with a diversity of county pairs \extended{(Table \ref{tab:h5_data_stats})}.
Furthermore, we conduct sensitivity analyses with $h=4$ and $h=6$ and show that results remain highly similar \extended{(Figure \ref{fig:bandwidth_results})}.

\paragraph{Loss-corrected negative sampling.}
To make estimation computationally feasible in this large-scale setting, we perform negative sampling. 
Specifically, for each zero data point $(i, j, w)$, we define its sampling probability $s_{ijw}$ as inversely proportional to the distance between the CBG and POI  ($s_{ijw} \propto \frac{1}{1 + d_{ij}}$). We do this to upweight ``hard'' negative samples; that is, since far-apart CBGs and POIs are highly unlikely to have any visits, the model learns more from nearby CBGs and POIs with zero visits.
% \extended{Then, we scale $s_{ijw}$ such that, on expectation, we sample a fixed percentage (e.g., 2\%) of the zero data points in each week.} 
However, a unique aspect of our problem---which does not typically appear in other machine learning prediction problems where negative sampling might be used, such as link prediction or learning word embeddings---is that because we seek to interpret the model parameters as effect sizes, our learned model parameters need to be unbiased estimates of the model parameters when learned on the full data.
Left uncorrected, negative sampling biases our model parameters by greatly reducing the number of zeros in the training data.

In the Appendix we show that by weighting each sampled zero data point by $\frac{1}{s_{ijw}}$ when computing the overall loss (negative log likelihood), our stochastic gradient (which is stochastic from sampling) forms an unbiased estimate of the true gradient, which ultimately guarantees unbiased parameter estimates assuming proper model specification. We also show that upweighting harder negative samples, as well as increasing the size of the sample, decreases the variance of the stochastic gradient, providing formal validation of these techniques.
In our experiments, we retain 2\% of the zero data points, with sampling probabilities inversely weighted by distance. We verify that after incorporating our loss corrections, different negative sampling schemes arrive at the same average parameters, but distance-weighting and larger samples decrease variance. The agreement between the estimates from different negative sampling schemes is consistent with the underlying model being properly specified.
% We also incorporate uncertainty from negative sampling into our procedure for building confidence intervals, which we describe below.

\paragraph{Uncertainty quantification with bootstrapping.}
We run 30 trials, where in each trial, we perform negative sampling on the zero data points and we sample $N_{nnz}$ non-zero data points with replacement, where $N_{nnz}$ is our total number of non-zero data points. For a given estimand, such as $\tau_{PR} = \exp(\beta_{PR} - \beta_{PP})$, we compute its 95\% confidence interval as $\bar{\tau}_{PR} \pm 1.96 \cdot \hat{\sigma}_{\tau_{PR}}$, where $\bar{\tau}_{PR}$ and $\hat{\sigma}_{\tau_{PR}}$ are its sample mean and standard deviation over trials, respectively. This procedure captures uncertainty from the data and from negative sampling, although we show that, given our chosen negative sampling scheme, the former accounts for the vast majority of the variance \extended{(Figure \ref{fig:neg_sample_cis})}.

==> Spillovers paper - arxiv/conclusion.tex <==
\section{Conclusion}
Geographic spillovers arise in many domains, but there are few opportunities to reliably estimate spillover effects.
In this work, we identify a novel setting that is uniquely suitable for spillover analysis, California's Blueprint for a Safer Economy, which defined a set of policies applied with the same deterministic thresholds across 58 counties.
We leverage these properties to develop a causal inference framework that allows us to make unconfounded estimates of spillover movement between counties and we observe significant spillovers in many POI groups. Finally, we evaluate the cost of spillovers on policies across spatial scales, analyzing the trade-off between efficacy and flexibility.
% Our approach furthermore enables us to analyze the consequences of spillovers on higher-level policy decisions, as we demonstrate that county-level restrictions can only achieve 62\% of the mobility reduction that would be achieved by statewide restrictions. 

Our work is not without limitations. First, SafeGraph's data does not cover all POIs or populations uniformly. To mitigate this issue, we control for CBG weekly device count, only estimate effects for the largest POI categories, and drop categories such as elementary schools that have unreliable coverage from cell phone apps. 
Second, our causal inference framework may not entirely satisfy SUTVA, the assumption that a unit's outcome is only influenced by its own treatment. 
In this work, we attempt to better satisfy SUTVA by modeling the effect of pairwise policies on cross-county movement, instead of only modeling the effect of a single county's policies on its population's mobility, as prior work has done. 
However, future work should explore interference beyond pairs; for example, mobility from county $A$ to $B$ may depend not only on $A$ and $B$'s policies but also on the policies of $A$'s other neighbors.
We also hope that future work will dive deeper into the complex trade-offs of policymaking for interconnected regions. 
In this work, we explored efficacy and flexibility, but other dimensions should be considered, such as
% In this work, we demonstrated that due to spillovers, local policies can be substantially less effective than global policies, since populations can cross borders to circumvent restrictions. 
% However, local policies also provide flexibility, such as not requiring the entire state to shut down (which incurs serious economic costs) when only a few counties have outbreaks.
% We hope to explore further dimensions of this trade-off, such as 
equity in the context of certain regions bearing disproportionate risks and unequal resources (e.g., with resourced areas better able to handle spikes in COVID-19 cases).
% As many of the world's most urgent challenges---e.g., climate change, global pandemics---involve policy planning across heterogeneous and interconnected regions, we hope that our work and future directions will guide more effective and equitable policymaking in the face of spillovers.

==> Spillovers paper - arxiv/data.tex <==
\section{Data} \label{sec:data}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/fig1.pdf}
    \caption{Primary data sources. (a) Percentage of California counties in Blueprint tiers---purple, red, orange, and yellow---over time (greyed-out period represents Regional Stay-At-Home Order); (b) Tiers in the week of March 15, 2021; (c) Average weekly visits per device over time.}
    \label{fig:data_plots}
\end{figure}

\paragraph{California Blueprint for a Safer Economy.}
The Blueprint was implemented for all 58 counties in California from August 30, 2020 to June 15, 2021. It consisted of four tiers: purple (``widespread''), red (``substantial''), orange (``moderate''), and yellow (``minimal''). These tiers corresponded to mobility policies of decreasing restrictiveness; for example, in the purple tier, most non-essential indoor businesses were closed, while in yellow, they could be open with modifications.
% To advance to a less restricted tier, counties needed to meet the pre-determined thresholds for COVID-19 case rate and test positivity.
% (see Section \ref{sec:tier_assignment} for a detailed discussion of the Blueprint's tier assignment rules). 
We use the archived data sheets from the California Department of Public Health (CDPH), which provide detailed documentation of every county's weekly tier assignment and the COVID-19 metrics used to make those assignments.\footnote{\url{https://www.cdph.ca.gov/Programs/CID/DCDC/Pages/COVID-19/CaliforniaBlueprintDataCharts.aspx}}
% At the start of each week (on Monday), CDPH assessed COVID-19 metrics from the prior weeks to determine each county's tier for the coming week. New tiers were announced on Tuesday and became effective on Wednesday. 
In Figure \ref{fig:data_plots}a, we visualize the progression of counties through tiers over time; we grey out the period from December 5, 2020 to January 25, 2021, during which most of the state was under a Regional Stay-At-Home Order \citep{cdph2020stayathome}. 
We can see that counties generally moved through similar tiers at similar times, which is expected, since COVID-19 severity was correlated across counties. 
However, in many weeks, we also see substantial representation from at least two different tiers. For example, in the week of March 15, 2021, there were 11 counties in the purple tier, 42 in the red tier, 4 in the orange tier, and 1 in the yellow tier (Figure \ref{fig:data_plots}b). Many of these differing tiers appeared between adjacent counties, enabling the analysis of spillovers across county borders.


\paragraph{Mobility network.} 
We use data from SafeGraph, a company that anonymizes and aggregates location data from mobile apps.
For each POI, SafeGraph provides weekly estimates of where visitors are coming from, aggregated over CBGs.\footnote{\url{https://docs.safegraph.com/docs/weekly-patterns}} 
This creates a dynamic, bipartite graph between CBGs and POIs, where an edge weight $Y_{ijw}$ represents the number of visits recorded by SafeGraph from CBG $c_i$ to POI $p_j$ in week $w$. SafeGraph also reports how many devices they recorded in each CBG and week. Incorporating device counts into our model allows us to account for varying coverage across CBGs and over time.

In Figure \ref{fig:data_plots}c, we show the average number of weekly visits recorded per device over time, aggregated over the entire CBG-POI network for California. We see that visits increased post-Regional Stay-at-Home as Blueprint tiers decreased in restrictiveness. 
However, various latent variables could explain this correlation, such as reduced COVID-19 severity leading to less restrictive tiers
% , an increased understanding of COVID-19 transmission mechanisms, 
and less fear of visiting places. 
Thus, it is necessary to develop a robust causal framework that allows us to disentangle tier effects from confounders, which we describe in the following section.

% TODO - stats on number of POIs and CBGs 




==> Spillovers paper - arxiv/intro.tex <==
\section{Introduction}
Many policies in the United States---COVID-19 restrictions, environmental regulations, and laws controlling the sales of e-cigarettes, firearms, and controlled substances---are determined at the state- or county-level.
Local policy regimes provide flexibility between regions, allowing policymakers to set regulations depending on local circumstances (e.g., COVID-19 severity) and the preferences of their constituents (e.g., on gun control).
On the other hand, allowing policies to be set locally often results in differing levels of restrictiveness between neighboring regions. These differences can lead to \textit{geographic spillovers}, where populations circumvent restrictions by traveling to less restricted regions nearby. 
Spillovers risk undermining the efficacy of local policies; for example, if banned goods are imported across state borders or if, during the pandemic, individuals in counties under lockdown continue to visit places in neighboring counties.
% For example, due to porous state borders, populations may import illicit substances or firearms, which is known as \textit{border trade}.
Furthermore, spillovers can affect important downstream consequences. For example, the movement of individuals from more restricted (and possibly more infected) regions to less restricted (and possibly less infected) regions during the pandemic could result in greater overall spread of the virus.
% Thus, understanding spillovers is key to policy planning for interconnected regions.

However, there are few opportunities to reliably estimate causal spillover effects.
Researchers cannot run experiments to randomly assign policies to states and counties, and causal identification is difficult in most observational studies, due to the presence of confounders. For example, attempting to study the effects of COVID-19 restrictions (e.g., closing restaurants) on mobility patterns introduces potential confounding covariates that predict both the treatment and the outcome, such as current COVID-19 severity in the region and the population's demographics. 
Prior work has attempted to address these confounders by controlling for them, but there could always be unobserved or unknown confounders that bias causal estimates.
Furthermore, the decentralized nature of policymaking that gives rise to potential spillovers also often results in varying policy definitions and implementations across regions.
This heterogeneity makes it difficult to define a consistent treatment whose effects we can measure.

In this work, we introduce a setting in which we can make unconfounded estimates of the spillover effects of consistent policies.
We focus on California's Blueprint for a Safer Economy, a statewide policy framework that determined weekly county-level mobility restrictions for all 58 counties in California from August 2020 to June 2021.
The Blueprint consisted of four tiers that corresponded to policies of decreasing restrictiveness. 
At the start of each week, each county’s tier was determined based on that county's COVID-19 metrics (case rate and test positivity) in the preceding weeks.
The California Blueprint presents a unique opportunity for studying spillover for three reasons: (1) neighboring counties were frequently in differing tiers, enabling the analysis of spillovers from more restricted to less restricted counties; (2) tiers were defined in the same way across counties, yielding a consistent treatment; (3) tiers were deterministically assigned at the thresholds of COVID-19 metrics. These three ingredients allow us to develop a causal inference framework based on regression discontinuity design to make unconfounded estimates of spillover effects.

To capture spillover, we focus on cross-county mobility in a large-scale mobility network. 
Our network is a dynamic bipartite graph that represents the weekly movements of individuals from census block groups (CBGs) to specific points-of-interest (POIs) such as restaurants and grocery stores. 
Our objective is to estimate the effect of pairwise county tiers on the number of visits from each CBG to POI. 
The mobility network for California contains around 23,000 CBGs and 130,000 POIs, with nearly 3 billion edges per week. 
We use stochastic gradient descent, with loss-corrected negative sampling, to make estimation computationally feasible in this large-scale setting.
Studying mobility patterns at the POI-level enables us to estimate heterogeneous treatment effects for POI categories; this ability is particularly relevant since tier restrictions were often industry-specific.
% Furthermore, studying CBG-POI visits allows us to include more precise covariates in our model, such as CBG demographics and the distance between POIs and CBGs, which would be ill-defined at the county-level. 
% Finally, our fitted model is able to produce counterfactual CBG-POI mobility networks under different tier assignments, which are instrumental for downstream analyses.

Finally, our spillover estimates allow us to quantify the cost of spillovers on policies across spatial scales. 
In the presence of spillovers, we find that county-level restrictions are, on average, only 54\% as effective as statewide restrictions at reducing mobility.
However, intermediate strategies of macro-county restrictions---when counties are grouped intelligently---can balance the trade-off between the policy flexibility and efficacy.
We show that finding the most effective county partition for a given spatial granularity is equivalent to solving a minimum $k$-cut problem on an undirected county graph weighted by our spillover estimates.
Using this approach, we identify macro-county restrictions that recover over 90\% of statewide mobility reductions, while maintaining substantial flexibility between counties.

% With our spillover estimates, we are able to demonstrate how spillovers introduce tradeoffs for policymaking at different spatial scales.
% Compared to statewide policies that require all counties to have the same mobility restrictions, regardless of their COVID-19 severity, county-level policies offer substantially more flexibility. However, in the presence of spillovers, county-level policies may become far less effective, as outflow from more restricted to less restricted regions circumvent intended reductions in mobility and mixing. 
% In the final section of our paper, we formalize the tradeoff between flexibility and efficacy for a given policy (i.e., partition of counties) and use our spillovers estimates to quantify the cost of spillovers. We show that while county-level restrictions are only half as effective as statewide restrictions at reducing population mobility, macro-county restrictions can 

% In the presence of spillovers, we find that county-level restrictions are, on average, only 53\% as effective as statewide restrictions at reducing population mobility; however, macro-county restrictions can recover over 90\% of statewide mobility reductions when county partitions are optimized. We show that finding the most effective county partition for a given spatial granularity is equivalent to solving the minimum $k$-cut problem on an undirected county graph weighted by our spillover estimates, and, by computing these partitions for a variety of spatial granularities, we can evaluate the trade-off between the efficacy and flexibility of policies.
% For example, our counterfactual networks may be combined with existing models that rely on fine-grained mobility patterns; for example, with state-of-the-art epidemiological models \citep{chang2020covid} to more realistically estimate the impacts of policy interventions on COVID-19 outcomes.

In summary, our contributions are as follows:
\begin{itemize}
    \item \textbf{Setting:} we identify a novel setting for studying spillovers where the same set of policies was applied with the same thresholds to many areas;
    \item \textbf{Methods:} we develop a regression discontinuity (RD) design framework that allows us to make unconfounded estimates of heterogeneous spillover effects in this setting, estimated over a large-scale mobility network containing billions of edges;
    \item \textbf{Analyses:} we demonstrate significant spillover effects in many POI groups and evaluate the costs of these spillovers on policies across spatial scales.
\end{itemize}
In a complex, interconnected world with few opportunities to reliably estimate policy effects, our work is among the first to identify a setting where spillovers can be rigorously estimated and to develop an appropriate methodology to estimate and evaluate the effects of spillovers.\footnote{The code to run our experiments and regenerate figures is available at \url{https://github.com/snap-stanford/covid-spillovers}. 
We also provide our constructed $Z$ variables (Section \ref{sec:causal}) that can be used with RD design to estimate the effects of the California Blueprint tiers on spillovers and other outcomes.
}

% Finally, studying CBG-POI visits instead of county-county visits increases our data size by 900,000$\times$. Our mobility network for California contains approximately 23,000 CBGs and 130,000 POIs, with nearly 3 billion edges in a single week (while there are 58 counties). 
% Having such large data counteracts one of the primary drawbacks of RD design, which limits analysis to data points within a narrow margin of the threshold(s) upon which treatment is determined. As a result of this data loss, RD designs often suffer from wide confidence intervals. 
% In this case, however, we still retain millions of data points in our analysis, with narrow CIs even after we apply corrections for multiple hypothesis testing. 
% This is especially important when analyzing the effects of COVID-19 restrictions on mobility, where prior studies have shown small effect sizes; for example, estimating that complete lock-downs at the beginning of the pandemic only contributed to a XX\% reduction in mobility. Here, we should expect even smaller effect sizes, as we are studying changes in cross-county mobility from switching from adjacent tiers (within a 4-tier system) months into the pandemic.
% Thus, by combining our RD-based causal framework and massive mobility network, we introduce a rare opportunity to estimate rigorous, heterogeneous, and still significant spillover effects.


==> Spillovers paper - arxiv/related_work.tex <==
\section{Related Work}
Spillovers often arise from decentralized policymaking for interconnected regions. 
For example, \citet{sigman2005environmental} finds that water quality is lower at stations downstream of states that are authorized to control their own water programs, since they ``free-ride.'' \citet{coates2017guns} show that in states with stronger gun laws, there is an increased likelihood of gun imports from states with weaker gun laws. 
\citet{bronars1998guns} show that while a concealed handgun law led to a reduction in crime in the state, it also led to an increase in crimes in neighboring states, suggesting that criminals were crossing borders.
\citet{hao2017marijuana} find that legalization of recreational marijuana in a state leads to an increase in marijuana-related arrests in bordering states. 
Spillovers also arise in online contexts, where instead of crossing geographic borders, users can migrate across platforms if they are banned on one platform; furthermore, levels of toxicity and radicalization are sometimes higher on the new, often less regulated platforms, compromising the efficacy of the original content moderation \citep{ribeiro2021content, ali2021deplatforming}. 
% Relatedly, studies have also shown that policies themselves (not only population behavior) are subject to spillovers; for example, with spillover effects on state spending \citep{baicker2005spending, case1993budget}.

In the context of COVID-19, prior research has mostly focused on the direct effects of policies on population health or behavior, without explicitly modeling spillovers \citep{chernozhukov2021causal, nguyen2020mobility, brauner2020science}. \citet{chandrasekhar2021interacting} investigate disease spillovers between interconnected regions in a model-based setting and \citet{holtz2020interdependence} provide early evidence of mobility spillovers, showing that a state's population reduced its own mobility when neighboring states implemented shelter-in-place policies. Most related to our work is \citet{zhao2021spillovers}, who use a difference-in-difference approach to estimate the effects of COVID-19 policies on mobility and provide evidence of spillovers in cross-state travel. We build on this work by addressing two primary limitations of their study: first, the authors note that their estimates could be confounded by unobserved, time-varying factors; other research on spillovers also suffers from potential confounding, using difference-in-difference approaches \citep{hao2017marijuana, holtz2020interdependence} or regressions \citep{coates2017guns, sigman2005environmental, bronars1998guns}. 
Second, in order ``to create sufficient statistical power to identify causal effects,'' the authors collapse different policy interventions into general policy ``types'' (e.g., resuming dine-in and lifting gathering restrictions are both counted as reopening), which violates assumptions of consistent treatment.

In contrast with prior work, we are able to identify unconfounded spillover estimates for a single set of policies by applying our RD-based framework to California's Blueprint for a Safer Economy. 
Furthermore, by estimating effects on the CBG-POI network, our model enables the analysis of counterfactual fine-grained mobility patterns under different pandemic policies. 
Understanding mobility patterns has been essential to controlling the spread of COVID-19 \citep{buckee2020aggregated}, and many researchers rely on fine-grained mobility data to model the effect of mobility on the spread of the virus \citep{badr2020mobility, chinazzi2020, kraemer2020mobility, chang2020covid, chang2021kdd, nouvellet2021reduction}.
Our model furthers such analyses by investigating the complex effects of policy interventions on mobility, closing the gap from policy to behavior to COVID-19 outcomes.

==> Spillovers paper - arxiv/results.tex <==
\section{Results}
\label{sec:results}
\paragraph{Spillover estimates.}
\extended{We learn heterogeneous effects for different POI groups, where we consider all ``top''-categories (first 4 digits of the POI's NAICS code) with at least 1000 POIs.\footnote{Following prior work using SafeGraph data \citep{chang2020covid}, we drop the category ``Elementary and Secondary Schools'' due to poor coverage of children from cell phone data.}
We also include separate effects for 4 ``sub''-categories (first 6 digits) of interest, all of which have over 1000 POIs. In Table \ref{tab:poi-groups}, we provide the NAICS codes, descriptions, and number of POIs in each POI group.}

We present our spillover results in Figure \ref{fig:spillover_results}.
% , with heterogeneous effects learned for different POI groups.
First, we find significant positive $PR$ effects in 21 out of 24 groups (all results remain significant with Bonferroni correction). That is, visits from the CBG increase significantly when the POI's county changes from purple to red, while the CBG's county remains in purple. This indicates spillovers, as people from more restricted counties spill over in less restricted, adjacent counties. 
Furthermore, we observe varying effect sizes; for example, with larger effects in retail (General Merchandise Stores, Automotive Stores, Clothing Stores, Building Material and Supplies Dealers, Department Stores), most eating places (Snack Bars, Full-Service Restaurants, Drinking Places), and gyms (Fitness and Recreational Sports Centers). 
Smaller effects are in essential retail (Grocery Stores, Gas Stations), hotels (Traveler Accommodation), malls (Lessors of Real Estate), museums, historical sites, and nature parks (Museums, Historical Sites, and Similar Institutions).
\extended{This heterogeneity in effect size may partially reflect differences across sectors in tier restrictions. For example, essential retail, hotels, and malls remained open indoors with modifications under both tiers, while restaurants and gyms---which have larger estimated spillovers---were outdoor only under the purple tier and open indoors with modifications under the red tier (Table \ref{tab:blueprint_sector}).}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/fig3.pdf}
    \caption{Estimated spillover effects across POI groups, with 95\% confidence intervals.}
    \label{fig:spillover_results}
\end{figure}

We also observe significant positive $RR$ effects in 22 POI groups (21 with Bonferroni correction), as in, visits increase significantly when both the CBG and POI are in red, compared to when they are both in purple. Furthermore, in most POI groups, the $PR$ effect is \textit{larger} than the $RR$ effect (although not always significantly so). This suggests an interaction effect: individuals not only spill over into adjacent counties when those counties become less restrictive, but also the spillover is larger if their home counties are more restrictive. 
Finally, we observe a varying effect of $RP$, which represents when the CBG changes from purple to red, while the POI remains in purple. The effect is slightly positive or negative for some POI groups, but significant in neither direction for most. We hypothesize that two mechanisms take place here: on one hand, since the POI is in a more restricted tier than the CBG, it becomes less appealing; on the other hand, since the CBG opened up, its population is more willing to travel. These counteracting mechanisms may explain the varying and weak $RP$ effects across POI groups. 

\paragraph{Local vs. global restrictions.}
To contrast local and global approaches to policymaking, we use our fitted model to compare counterfactual mobility reductions under county-level vs. hypothetical statewide restrictions.
Formally, let $\mathbf{T} \in \mathbb{R}^{58}$ represent the treatment vector for all counties. For each county $A$, we estimate this county's expected mobility (out-degree in the mobility network) under three treatment conditions: when the entire state is in the red tier ($\mathbf{T}_R$), when the entire state is in the purple tier ($\mathbf{T}_P$), and when only this county is in purple while the rest of the state remains in red ($\mathbf{T}_A$). 
We then compare the mobility reduction that a county would experience by going to purple on its own, relative to the statewide shutdown, where all counties go to purple:
\begin{align}
    r(A) &= \frac{\mathbb{E}[out(A) | \mathbf{T}_R] - \mathbb{E}[out(A) | \mathbf{T}_A]}{\mathbb{E}[out(A) | \mathbf{T}_R] - \mathbb{E}[out(A) | \mathbf{T}_P]}.
\end{align}
We calculate $\mathbb{E}[out(A) | \mathbf{T}]$ as the sum over within-county visits and out-of-county visits:
\begin{align}
    \mathbb{E}[out(A) | \mathbf{T}] =  \mathbb{E}[Y_{AA} | T_A] + \hspace{-2mm} \sum_{B \in N(A)} \mathbb{E}[Y_{AB} | T_A, T_B],
\end{align}
where $Y_{AB}$ represents the total number of visits from any CBG in county $A$ to any POI in county $B$. When we use our fitted model to compute the conditional expectation of $Y_{AB}$ given tiers, we assume $Z = 0$ for all CBGs and POIs, since our RD-based framework estimated tier effects at the joint cutoff. We also marginalize over the remaining dynamic covariate, the CBG's weekly device count, by taking each CBG's average device count \extended{over the 9-week period that we study. 
In the Appendix, we describe how to efficiently compute $Y_{AB}$ for all pairs of counties and possible tier pairs.}

We estimate that counties applying local restrictions can only achieve, on average, 
54.0\% (46.4\%--61.7\%) of the reduction in mobility that they would experience under a statewide shutdown. 
\extended{Small counties are particularly affected, keeping only 41.7\% (31.0\%--52.4\%) of their statewide mobility reduction, while large counties retain 62.1\% (56.3\%--67.9\%).}
While we assume that the reduction in mobility \textit{within} the county stays the same between local and global regimes, the difference arises from the increase in \textit{out-of-county visits} when all surrounding counties are less restricted in the red tier; \extended{this is why smaller counties are especially hard-hit, since a larger fraction of their mobility tends to be out-of-county}.
We also consider a less extreme case, where instead of having all surrounding counties in red, we use the actual configuration of tiers from the Blueprint. We still observe serious costs to efficacy in these more realistic settings: over the course of our study period, as the number of counties in purple fell from 40 to 11 to 3, the average percent of mobility reduction kept for counties in purple (compared to statewide shutdown) fell from 94\% to 75\% to 65\% \extended{(Figure \ref{fig:rwa_over_real_tiers})}.
These substantial decreases in efficacy demonstrate the cost of spillovers on local policies.

\paragraph{Balancing efficacy and flexibility.} 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/fig4.pdf}
    \caption{Macro-county restrictions. (a) Actual macro-counties from California's Stay-At-Home Order. (b) Trade-off between flexibility (lower macro-county size) versus efficacy (higher $r_M(A)$), with 95\% confidence intervals. (c) Macro-county partition for $k=7$, computed by METIS.}
    \label{fig:pareto_curve}
\end{figure}

Although local policies are less effective in the presence of spillovers, global policies are often too blunt and inflexible. In our final analysis, we explore this trade-off between efficacy and flexibility across policies at different spatial scales. Instead of being entirely local (county-level) or global (statewide), intermediate strategies could be implemented at the macro-county level. California in fact pursued such a strategy with its Regional Stay-At-Home Order \citep{newsom2020stayathome} that grouped counties into 5 macro-counties, each containing 11--13 counties (Figure \ref{fig:pareto_curve}a). 
Given a county partition $M$, we extend our analysis to compute $r_M(A)$, the ratio of mobility reduction that each county $A$ would experience if only its \textit{macro-county} went to purple, compared to statewide shutdown.
% \begin{align}
%     r_M(A) &=  \frac{\mathbb{E}[out(A) | \mathbf{T}_R] - \mathbb{E}[out(A) | \mathbf{T}_{M(A)}]}{\mathbb{E}[out(A) | \mathbf{T}_R] - \mathbb{E}[out(A) | \mathbf{T}_P]}.
% \end{align}
When we use the county partition from California's Regional Stay-At-Home Order, we find that macro-county restrictions can achieve 92.1\% (90.9\%--93.3\%) of statewide mobility reductions. In contrast, if we use a random partitioning of counties into equal-sized segments, such restrictions only reach 62.3\% (54.3\%--70.4\%, 95\% CI includes randomness in partitioning) of statewide reductions. Thus, policies of intermediate scale are promising in their ability to balance efficacy and flexibility, but achieving that balance relies on optimizing how macro-counties are defined.

Given a desired number of macro-counties $k$, we show in the Appendix that we can find the optimal county partition that maximizes the average $r_M(A)$ over counties by solving a minimum $k$-cut problem, which seeks to partition the nodes of an undirected graph into $k$ disjoint sets while minimizing the total weight of edges between nodes in different sets.
We define our undirected graph as one between counties, where the edge weight $w_{AB}$ between two adjacent counties $A$ and $B$ is
\begin{align}
    w_{AB} = &\frac{\mathbb{E}[Y_{AB} | P,R] - \mathbb{E}[Y_{AB} | P,P]}{\mathbb{E}[out(A) | \mathbf{T}_R] - \mathbb{E}[out(A) | \mathbf{T}_P]} + \\
    &\frac{\mathbb{E}[Y_{BA} | P,R] - \mathbb{E}[Y_{BA} | P,P]}{\mathbb{E}[out(B) | \mathbf{T}_R] - \mathbb{E}[out(B) | \mathbf{T}_P]} \nonumber.
\end{align}
To achieve evenly sized macro-counties, we impose an additional constraint (common in balanced graph partitioning) that each set is no larger than $1.05 \cdot \frac{N}{k}$, where $N=58$ is the total number of counties.
While this problem is NP-hard, we can approximate the solution using METIS \citep{karypis1997metis}.
In Figure \ref{fig:pareto_curve}b, we display our solutions over a range of $k$. Smaller macro-county sizes are preferred for flexibility (x-axis), while higher $r_M(A)$ represents better efficacy (y-axis). We observe a clear trade-off between the two objectives; however, even small macro-counties---when grouped intelligently---yield large improvements in efficacy over county-level restrictions. For example, by just increasing the average macro-county size to 8 (still $1/7^{th}$ the total number of counties), we reach over 90\% of the full efficacy of the much more drastic statewide shutdown (Figure \ref{fig:pareto_curve}c).
